Planning 5G Networks for Rural Fixed Wireless Access

We study the planning of a rural 5G multi-user massive MIMO fixed wireless access system to offer fixed broadband service to homes. Specifically, we aim to determine the user limit, i.e., the maximum number of homes that can simultaneously receive target minimum bit rates (MBRs) on the downlink (DL) and on the uplink (UL) given a set of network resources and a cell radius. To compute that limit, we must understand how resources should be shared between the DL and UL and how user and stream selection, precoding and combining, and power distribution should be performed. We use block diagonalization and propose a static grouping strategy that organizes homes into fixed groups (of possibly different sizes) in the DL and UL; then we develop a simple approach to compute the user limit that we validate numerically. We study the impact of group size and show that smaller groups yield larger user limits in a 3.5 GHz band. We show how the user limit at different cell radii is impacted by the system bandwidth, the number of antennas at the base station and homes, the transmit power, and the DL and UL MBRs. Lastly, we offer insights into how the network could be operated.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> bibtex/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> bibtex/bib/old_with_dois.tex <==
@ARTICLE{larsson2014mimo,
  author={E. G. {Larsson} and O. {Edfors} and F. {Tufvesson} and T. L. {Marzetta}},
  journal=IEEE_M_COM, 
  title={{Massive MIMO for Next Generation Wireless Systems}}, 
  month=feb,
  year={2014},
  volume={52},
  number={2},
  pages={186-195},
  doi={10.1109/MCOM.2014.6736761}}

@ARTICLE{shafi2017tutorial,
  author={M. {Shafi} and A. F. {Molisch} and P. J. {Smith} and T. {Haustein} and P. {Zhu} and P. {De Silva} and F. {Tufvesson} and A. {Benjebbour} and G. {Wunder}},
  journal=IEEE_J_JSAC, 
  title={{5G: A Tutorial Overview of Standards, Trials, Challenges, Deployment, and Practice}}, 
  month=jun,
  year={2017},
  volume={35},
  number={6},
  pages={1201-1221},
  doi={10.1109/JSAC.2017.2692307}}

@ARTICLE{kaltenberger2009mimo,
  author={F. {Kaltenberger} and M. {Kountouris} and D. {Gesbert} and R. {Knopp}},
  journal=IEEE_J_WCOM, 
  title={{On the Trade-Off Between Feedback and Capacity in Measured MU-MIMO Channels}}, 
  month=sep,
  year={2009},
  volume={8},
  number={9},
  pages={4866-4875},
  doi={10.1109/TWC.2009.081670}}
  
@ARTICLE{liu2012mimo,
  author={L. {Liu} and R. {Chen} and S. {Geirhofer} and K. {Sayana} and Z. {Shi} and Y. {Zhou}},
  journal=IEEE_M_COM, 
  title={{Downlink MIMO in LTE-Advanced: SU-MIMO vs. MU-MIMO}}, 
  month=feb,
  year={2012},
  volume={50},
  number={2},
  pages={140-147},
  doi={10.1109/MCOM.2012.6146493}}

@ARTICLE{aldubaikhy2020mmwave,
  author={Aldubaikhy, Khalid and Wu, Wen and Zhang, Ning and Cheng, Nan and Shen, Xuemin},
  journal=IEEE_M_WC, 
  title={{mmWave IEEE 802.11ay for 5G Fixed Wireless Access}}, 
  month=apr,
  year={2020},
  volume={27},
  number={2},
  pages={88-95},
  doi={10.1109/MWC.001.1900174}}

@ARTICLE{brighente2020modular,
  author={Brighente, Alessandro and Gambini, Jonathan and Tomasin, Stefano},
  journal=IEEE_J_COM, 
  title={{Modular Hybrid Beamforming for mmWave Fixed Wireless Access}}, 
  month=aug,
  year={2020},
  volume={68},
  number={8},
  pages={5145-5158},
  doi={10.1109/TCOMM.2020.2992470}}


@INPROCEEDINGS{colpaert2020fixed,
  author={Colpaert, Achiel and Vinogradov, Evgenii and Pollin, Sofie},
  booktitle={2020 IEEE 91st Vehicular Technology Conference (VTC2020-Spring)}, 
  title={{Fixed mmWave Multi-User MIMO: Performance Analysis and Proof-of-Concept Architecture}}, 
  month=may,
  year={2020},
  volume={},
  number={},
  pages={1-5},
  address={Antwerp, Belgium},
  doi={10.1109/VTC2020-Spring48590.2020.9128958}}

@INPROCEEDINGS{abozariba2019evaluating,
  author={Abozariba, Raouf and Davies, Eleanor and Broadbent, Matthew and Race, Nicholas},
  booktitle={2019 IEEE 2nd 5G World Forum (5GWF)}, 
  title={{Evaluating the Real-World Performance of 5G Fixed Wireless Broadband in Rural Areas}}, 
  month=sep,
  year={2019},
  volume={},
  number={},
  pages={465-470},
  address={Dresden, Germany},
  doi={10.1109/5GWF.2019.8911655}}

@ARTICLE{jaber2015tutorial,
  author={Jaber, Mona and Dawy, Zaher and Akl, Naeem and Yaacoub, Elias},
  journal=IEEE_O_CSTO, 
  title={{Tutorial on LTE/LTE-A Cellular Network Dimensioning Using Iterative Statistical Analysis}}, 
  month={2nd Quart.},
  year={2016},
  volume={18},
  number={2},
  pages={1355-1383},
  doi={10.1109/COMST.2015.2513440}}

@ARTICLE{taufique2017planning,
  author={Taufique, Azar and Jaber, Mona and Imran, Ali and Dawy, Zaher and Yacoub, Elias},
  journal={IEEE Access}, 
  title={{Planning Wireless Cellular Networks of Future: Outlook, Challenges and Opportunities}}, 
  year={2017},
  volume={5},
  number={},
  pages={4821-4845},
  doi={10.1109/ACCESS.2017.2680318}}

@ARTICLE{kaddoura2019greenfield,
  author={Kaddoura, Omar and Outes-Carnero, Jos{\'e} and Garc{\'i}a-Fern{\'a}ndez, Juan A. and Acedo-Hern{\'a}ndez, Rocio and Cer{\'o}n-Larrubia, Maria and R{\'i}os, Lorena and S{\'a}nchez-S{\'a}nchez, Juan J. and Barco, Raquel},
  journal=IEEE_J_COML, 
  title={{Greenfield Design in 5G FWA Networks}}, 
  month=dec,
  year={2019},
  volume={23},
  number={12},
  pages={2422-2426},
  doi={10.1109/LCOMM.2019.2939470}}

@ARTICLE{chiaraviglio2021planning,
  author={Chiaraviglio, Luca and Di Paolo, Cristian and Blefari Melazzi, Nicola},
  journal=IEEE_J_MC, 
  title={{5G Network Planning under Service and EMF Constraints: Formulation and Solutions}}, 
  year={2021},
  volume={},
  number={},
  pages={1-25},
  doi={10.1109/TMC.2021.3054482}}
  
@ARTICLE{khan2020service,
  author={Khan, M. Umar and Garc{\'i}a-Armada, A. and Escudero-Garz{\'a}s, J. J.},
  journal={IEEE Access}, 
  title={{Service-Based Network Dimensioning for 5G Networks Assisted by Real Data}}, 
  year={2020},
  volume={8},
  number={},
  pages={129193-129212},
  doi={10.1109/ACCESS.2020.3009127}}
 
@ARTICLE{kashef2016balanced,
  author={Kashef, Mohamed and Ismail, Muhammad and Serpedin, Erchin and Qaraqe, Khalid},
  journal=IEEE_J_JSAC, 
  title={{Balanced Dynamic Planning in Green Heterogeneous Cellular Networks}}, 
  month=dec,
  year={2016},
  volume={34},
  number={12},
  pages={3299-3312},
  doi={10.1109/JSAC.2016.2624098}}

@ARTICLE{ghazzai2015optimized,
  author={Ghazzai, Hakim and Yaacoub, Elias and Alouini, Mohamed-Slim and Dawy, Zaher and Abu-Dayya, Adnan},
  journal=IEEE_J_VT, 
  title={{Optimized LTE Cell Planning With Varying Spatial and Temporal User Densities}}, 
  month=mar,
  year={2016},
  volume={65},
  number={3},
  pages={1575-1589},
  doi={10.1109/TVT.2015.2411579}}

@INPROCEEDINGS{furqan2014effects,
  author={Furqan, Fatima and Hoang, Doan B. and Collings, Iain B.},
  booktitle={2014 IEEE 33rd International Performance Computing and Communications Conference (IPCCC)}, 
  title={{Effects of quality of service schemes on the capacity and dimensioning of LTE networks}}, 
  month=dec,
  year={2014},
  volume={},
  number={},
  pages={1-8},
  address={Austin, TX, USA},
  doi={10.1109/PCCC.2014.7017070}}

@INPROCEEDINGS{ng2012energy,
  author={Ng, Derrick Wing Kwan and Schober, Robert},
  booktitle={2012 IEEE International Conference on Communications (ICC)}, 
  title={{Energy-Efficient Resource Allocation in OFDMA Systems with Large Numbers of Base Station Antennas}}, 
  month=jun,
  year={2012},
  volume={},
  number={},
  pages={5916-5920},
  address={Ottawa, ON, Canada},
  doi={10.1109/ICC.2012.6364677}}

@ARTICLE{lima2013improved,
  author={Lima, Francisco Rafael Marques and Maciel, Tarcisio Ferreira and Freitas, Walter Cruz and Cavalcanti, Francisco Rodrigo Porto},
  journal=IEEE_J_VT, 
  title={{Improved Spectral Efficiency With Acceptable Service Provision in Multiuser MIMO Scenarios}}, 
  month=jul,
  year={2014},
  volume={63},
  number={6},
  pages={2697-2711},
  doi={10.1109/TVT.2013.2293333}}

@INPROCEEDINGS{zappone2015distributed,
  author={Zappone, Alessio and Sanguinetti, Luca and Bacci, Giacomo and Jorswieck, Eduard and Debbah, Mérouane},
  booktitle={2015 International Symposium on Wireless Communication Systems (ISWCS)}, 
  title={{Distributed Energy-Efficient UL Power Control in Massive MIMO with Hardware Impairments and Imperfect CSI}}, 
  month=aug,
  year={2015},
  volume={},
  number={},
  pages={311-315},
  address={Brussels, Belgium},
  doi={10.1109/ISWCS.2015.7454353}}

@ARTICLE{zappone2015energy,
  author={A. {Zappone} and L. {Sanguinetti} and G. {Bacci} and E. {Jorswieck} and M. {Debbah}},
  journal=IEEE_J_SP, 
  title={{Energy-Efficient Power Control: A Look at 5G Wireless Technologies}}, 
  month=apr,
  year={2016},
  volume={64},
  number={7},
  pages={1668-1683},
  doi={10.1109/TSP.2015.2500200}}

@ARTICLE{ho2008optimal,
  author={Ho, Winston W. L. and Liang, Ying-Chang},
  journal=IEEE_J_VT, 
  title={{Optimal Resource Allocation for Multiuser MIMO-OFDM Systems With User Rate Constraints}}, 
  month=mar,
  year={2009},
  volume={58},
  number={3},
  pages={1190-1203},
  doi={10.1109/TVT.2008.927721}}

@INPROCEEDINGS{elhajj2011dynamic,
  author={El Hajj, Ahmad M. and Dawy, Zaher},
  booktitle={2011 IEEE Global Telecommunications Conference - GLOBECOM 2011}, 
  title={{Dynamic Joint Switching Point Configuration and Resource Allocation in TDD-OFDMA Wireless Networks}}, 
  month=dec,
  year={2011},
  volume={},
  number={},
  pages={1-6},
  address={Houston, TX, USA},
  doi={10.1109/GLOCOM.2011.6133553}}

@ARTICLE{zorba2015energy,
  author={Zorba, Nizar and Verikoukis, Christos},
  journal=IEEE_J_SYST, 
  title={{Energy Optimization for Bidirectional Multimedia Communication in Unsynchronized TDD Systems}}, 
  month=jun,
  year={2016},
  volume={10},
  number={2},
  pages={797-804},
  doi={10.1109/JSYST.2015.2456072}}


@techreport{3gppTR38901,
    author = {{3GPP}},
    day = {11},
    institution = {{3rd Generation Partnership Project (3GPP)}},
    month = jan,
    year = {2020},
    note = {version 16.1.0},
    number = {38.901},
    title = {{5G; Study on channel model for frequencies from 0.5 to 100 GHz}},
    type = {Technical Report (TR)},
    url = {https://portal.3gpp.org/desktopmodules/Specifications/SpecificationDetails.aspx?specificationId=3173}
}

@ARTICLE{MacCartney2017,
  author={G. R. {MacCartney} and T. S. {Rappaport}},
  journal=IEEE_J_JSAC, 
  title={{Rural Macrocell Path Loss Models for Millimeter Wave Wireless Communications}}, 
  month=jul,
  year={2017},
  volume={35},
  number={7},
  pages={1663-1677},
  doi={10.1109/JSAC.2017.2699359}}
  
@ARTICLE{el2020accurate,
  author={Khaled, Zayan El and Ajib, Wessam and Mcheick, Hamid},
  journal={IEEE Access}, 
  title={{An Accurate Empirical Path Loss Model for Heterogeneous Fixed Wireless Networks Below 5.8 GHz Frequencies}}, 
  year={2020},
  volume={8},
  number={},
  pages={182755-182775},
  doi={10.1109/ACCESS.2020.3023141}}

@INPROCEEDINGS{schumacher2019coverage,
  author={Schumacher, Adrian and Merz, Ruben and Burg, Andreas},
  booktitle={2019 IEEE 89th Vehicular Technology Conference (VTC2019-Spring)}, 
  title={{3.5 GHz Coverage Assessment with a 5G Testbed}}, 
  month=apr,
  year={2019},
  volume={},
  number={},
  pages={1-6},
  address={Kuala Lumpur, Malaysia},
  doi={10.1109/VTCSpring.2019.8746551}}

@techreport{3gppTS381011,
    author = {{3GPP}},
    day = {24},
    institution = {{3rd Generation Partnership Project (3GPP)}},
    month = jan,
    year = {2020},
    note = {version 16.2.0},
    number = {38.101-1},
    title = {{5G; NR; User Equipment (UE) radio transmission and reception; Part 1: Range 1 Standalone}},
    type = {Technical Specification (TS)},
    url = {https://portal.3gpp.org/desktopmodules/Specifications/SpecificationDetails.aspx?specificationId=3283}
}

@techreport{3gppTS38211,
    author = {{3GPP}},
    day = {14},
    institution = {{3rd Generation Partnership Project (3GPP)}},
    month = jul,
    year = {2020},
    note = {version 16.2.0},
    number = {38.211},
    title = {{5G; NR; Physical channels and modulation}},
    type = {Technical Specification (TS)},
    url = {https://portal.3gpp.org/desktopmodules/Specifications/SpecificationDetails.aspx?specificationId=3213}
}

@techreport{3gppTS38213,
    author = {{3GPP}},
    day = {20},
    institution = {{3rd Generation Partnership Project (3GPP)}},
    month = jul,
    year = {2020},
    note = {version 16.2.0},
    number = {38.213},
    title = {{5G; NR; Physical layer procedures for control}},
    type = {Technical Specification (TS)},
    url = {https://portal.3gpp.org/desktopmodules/Specifications/SpecificationDetails.aspx?specificationId=3215}
}

@techreport{3gppTS38214,
    author = {{3GPP}},
    day = {20},
    institution = {{3rd Generation Partnership Project (3GPP)}},
    month = jul,
    year = {2020},
    note = {version 16.2.0},
    number = {38.214},
    title = {{5G; NR; Physical layer procedures for data}},
    type = {Technical Specification (TS)},
    url = {https://portal.3gpp.org/desktopmodules/Specifications/SpecificationDetails.aspx?specificationId=3216}
}

@ARTICLE{castaneda2016overview,
  author={Casta{\~n}eda, Eduardo and Silva, Ad{\~a}o and Gameiro, At{\'i}lio and Kountouris, Marios},
  journal=IEEE_O_CSTO, 
  title={{An Overview on Resource Allocation Techniques for Multi-User MIMO Systems}}, 
  month={1st Quart.},
  year={2017},
  volume={19},
  number={1},
  pages={239-284},
  doi={10.1109/COMST.2016.2618870}}

@ARTICLE{yoo2006optimality,
  author={Yoo, Taesang and Goldsmith, Andrea},
  journal=IEEE_J_JSAC, 
  title={{On the Optimality of Multiantenna Broadcast Scheduling Using Zero-Forcing Beamforming}}, 
  month=mar,
  year={2006},
  volume={24},
  number={3},
  pages={528-541},
  doi={10.1109/JSAC.2005.862421}}

@ARTICLE{zu2013generalized,
  author={Zu, Keke and de Lamare, Rodrigo C. and Haardt, Martin},
  journal=IEEE_J_COM, 
  title={{Generalized Design of Low-Complexity Block Diagonalization Type Precoding Algorithms for Multiuser MIMO Systems}}, 
  month=oct,
  year={2013},
  volume={61},
  number={10},
  pages={4232-4242},
  doi={10.1109/TCOMM.2013.090513.130038}}

@ARTICLE{spencer2004zero,
  author={Spencer, Q.H. and Swindlehurst, A.L. and Haardt, M.},
  journal=IEEE_J_SP, 
  title={{Zero-Forcing Methods for Downlink Spatial Multiplexing in Multiuser MIMO Channels}}, 
  month=feb,
  year={2004},
  volume={52},
  number={2},
  pages={461-471},
  doi={10.1109/TSP.2003.821107}}

@ARTICLE{chae2008block,
  author={Chae, Chan-Byoung and Shim, Seijoon and Heath, Robert W.},
  journal=IEEE_J_WCOM, 
  title={{Block Diagonalized Vector Perturbation for Multiuser MIMO Systems}}, 
  month=nov,
  year={2008},
  volume={7},
  number={11},
  pages={4051-4057},
  doi={10.1109/T-WC.2008.070262}}

@ARTICLE{liu2008cautious,
  author={Liu, Jianhua},
  journal=IEEE_J_VT, 
  title={{Be Cautious When Using the FIR Channel Model With the OFDM-Based Communication Systems}}, 
  month=mar,
  year={2009},
  volume={58},
  number={3},
  pages={1607-1612},
  doi={10.1109/TVT.2008.928897}}

@ARTICLE{zhang2021joint,
  author={Zhang, Yuhao and Mitran, Patrick and Rosenberg, Catherine},
  journal=IEEE_J_COM, 
  title={{Joint Resource Allocation for Linear Precoding in Downlink Massive MIMO Systems}}, 
  month=may,
  year={2021},
  volume={69},
  number={5},
  pages={3039-3053},
  doi={10.1109/TCOMM.2021.3053040}}

@INPROCEEDINGS{ying2014kronecker,
  author={Ying, Dawei and Vook, Frederick W. and Thomas, Timothy A. and Love, David J. and Ghosh, Amitava},
  booktitle={2014 IEEE International Conference on Communications (ICC)}, 
  title={{Kronecker product correlation model and limited feedback codebook design in a 3D channel model}}, 
  month=jun,
  year={2014},
  address={Sydney, NSW, Australia},
  volume={},
  number={},
  pages={5865-5870},
  doi={10.1109/ICC.2014.6884258}}

@ARTICLE{lim2017bounds,
  author={Lim, Hyeongyong and Jang, Yeonsoo and Yoon, Dongweon},
  journal=IEEE_J_WCOM, 
  title={{Bounds for Eigenvalues of Spatial Correlation Matrices With the Exponential Model in MIMO Systems}},
  month=feb,
  year={2017},
  volume={16},
  number={2},
  pages={1196-1204},
  doi={10.1109/TWC.2016.2641419}}

@INPROCEEDINGS{fan2013dual,
  author={Fan, Longfei and Li, Yabo and Zhao, Minjian},
  booktitle={2013 IEEE 24th Annual International Symposium on Personal, Indoor, and Mobile Radio Communications (PIMRC)}, 
  title={{Dual-polarized very large antenna array with exponential correlation matrix}}, 
  month=sep,
  year={2013},
  volume={},
  number={},
  pages={1386-1391},
  address={London, UK},
  doi={10.1109/PIMRC.2013.6666357}}

@INPROCEEDINGS{lagen2020new,
  author={Lagen, Sandra and Wanuga, Kevin and Elkotby, Hussain and Goyal, Sanjay and Patriciello, Natale and Giupponi, Lorenza},
  booktitle={ICC 2020 - 2020 IEEE International Conference on Communications (ICC)}, 
  title={{New Radio Physical Layer Abstraction for System-Level Simulations of 5G Networks}}, 
  month=jun,
  year={2020},
  volume={},
  number={},
  pages={1-7},
  address={Dublin, Ireland},
  doi={10.1109/ICC40277.2020.9149444}}

@INPROCEEDINGS{ikuno2010system,
  author={Ikuno, Josep Colom and Wrulich, Martin and Rupp, Markus},
  booktitle={2010 IEEE 71st Vehicular Technology Conference}, 
  title={{System Level Simulation of LTE Networks}}, 
  month=may,
  year={2010},
  volume={},
  number={},
  pages={1-5},
  address={Taipei, Taiwan},
  doi={10.1109/VETECS.2010.5494007}}

@INPROCEEDINGS{lopez2011optimization,
  author={L{\'o}pez-P{\'e}rez, David and Lad{\'a}nyi, {\'A}kos and J{\"u}ttner, Alp{\'a}r and Rivano, Herve and Zhang, Jie},
  booktitle={2011 Proceedings IEEE INFOCOM}, 
  title={{Optimization Method for the Joint Allocation of Modulation Schemes, Coding Rates, Resource Blocks and Power in Self-organizing LTE Networks}}, 
  month=apr,
  year={2011},
  volume={},
  number={},
  pages={111-115},
  address={Shanghai, China},
  doi={10.1109/INFCOM.2011.5934888}}

@ARTICLE{shen2006low,
  author={Zukang Shen and Runhua Chen and Andrews, J.G. and Heath, R.W. and Evans, B.L.},
  journal=IEEE_J_SP, 
  title={{Low Complexity User Selection Algorithms for Multiuser MIMO Systems With Block Diagonalization}}, 
  month=sep,
  year={2006},
  volume={54},
  number={9},
  pages={3658-3663},
  doi={10.1109/TSP.2006.879269}}

@INPROCEEDINGS{gupta2016rate,
  author={Gupta, Abhishek K. and Kulkarni, Mandar N. and Visotsky, Eugene and Vook, Frederick W. and Ghosh, Amitava and Andrews, Jeffrey G. and Heath, Robert W.},
  booktitle={2016 IEEE International Conference on Communications (ICC)}, 
  title={{Rate Analysis and Feasibility of Dynamic TDD in 5G Cellular Systems}},
  month=may,
  year={2016},
  volume={},
  number={},
  pages={1-6},
  address={Kuala Lumpur, Malaysia},
  doi={10.1109/ICC.2016.7511412}}

@INPROCEEDINGS{guo2018dynamic,
  author={Guo, Shaozhen and Hou, Xiaolin and Wang, Hanning},
  booktitle={2018 IEEE Wireless Communications and Networking Conference (WCNC)}, 
  title={{Dynamic TDD and Interference Management Towards 5G}}, 
  month=apr,
  year={2018},
  volume={},
  number={},
  pages={1-6},
  address={Barcelona, Spain},
  doi={10.1109/WCNC.2018.8377314}}

@inproceedings{ngo2013massive,
  author={Ngo, Hien Quoc and Larsson, Erik G. and Marzetta, Thomas L.},
  booktitle={2013 51st Annual Allerton Conference on Communication, Control, and Computing (Allerton)}, 
  title={{Massive MU-MIMO Downlink TDD Systems with Linear Precoding and Downlink Pilots}}, 
  month={Oct.},
  year={2013},
  volume={},
  number={},
  pages={293--298},
  address={Monticcello, IL},
  doi={10.1109/Allerton.2013.6736537}}

@INPROCEEDINGS{karlsson2014operation,
  author={Karlsson, Marcus and Larsson, Erik G.},
  booktitle={2014 IEEE 15th International Workshop on Signal Processing Advances in Wireless Communications (SPAWC)}, 
  title={{On the Operation of Massive MIMO with and without Transmitter CSI}}, 
  month=jun,
  year={2014},
  volume={},
  number={},
  pages={1-5},
  address={Toronto, ON},
  doi={10.1109/SPAWC.2014.6941305}}

@techreport{ericssonMIMO2018,
    institution = {{Ericsson}},
    author={{P. von Butovitsch \textit{et al.}}},
    month = {Nov.},
    year = {2018},
    title = {{Advanced antenna systems for 5G networks}},
    type = {White Paper},
    url = {https://www.ericsson.com/en/reports-and-papers/white-papers/advanced-antenna-systems-for-5g-networks}
}

@techreport{samsungMIMO2020,
    institution = {{Samsung}},
    month = {Dec.},
    year = {2020},
    title = {{Massive MIMO for New Radio}},
    type = {White Paper},
    url = {https://images.samsung.com/is/content/samsung/p5/global/business/networks/insights/white-papers/1208\_massive-mimo-for-new-radio/MassiveMIMOforNRTechnicalWhitePaper-v1.2.0.pdf}
}

@techreport{5gamericasMIMO2019,
    institution = {5G Americas},
    month = {Aug.},
    year = {2019},
    title = {{Advanced Antenna Systems for 5G}},
    type = {White Paper},
    url = {https://www.5gamericas.org/wp-content/uploads/2019/08/5G-Americas\_Advanced-Antenna-Systems-for-5G-White-Paper.pdf}
}
